Expansivity and unique shadowing

Let $f\colon X\to X$ be a continuous function on a compact metric space. We show that shadowing is equivalent to backwards shadowing and two-sided shadowing when the map $f$ is onto. Using this we go on to show that, for expansive surjective maps the properties shadowing, two-sided shadowing, s-limit shadowing and two-sided s-limit shadowing are equivalent. We show that $f$ is positively expansive and has shadowing if and only if it has unique shadowing (i.e.\ each pseudo-orbit is shadowed by a unique point), extending a result implicit in Walter's proof that positively expansive maps with shadowing are topologically stable. We use the aforementioned result on two-sided shadowing to find an equivalent characterisation of shadowing and expansivity and extend these results to the notion of $n$-expansivity due to Morales.

==> Sections/Graveyard/2ndWeakShadowing.tex <==
\section{Second weak shadowing} \label{section-second-weak}
In \cite{PiluginRodSakai2002} the authors introduce a property they call the second weak shadowing condition. A system has this property if pseudo-orbits contain true orbits in their neighbourhoods. In this section we show that any compact metric system exhibits this property. 


\begin{definition}
The system $(X,f)$ has the \textit{second weak shadowing} property if for all $\epsilon>0$, there exists 
$\delta>0$ such that for any $\delta$-pseudo-orbit $(x_i)_{i\in\omega}$, there exists a point $z$ such that

\[\Orb(z) \subseteq B_\epsilon\left( (x_i)_{i\in\omega}\right).\]
\end{definition}

Recall that the $\omega$-limit set of a point $x\in X$ is defined by
	\[\omega(x)\coloneqq \bigcap_{N \in \mathbb{N}}\overline{\{f^n(x) \mid n >N\}}.\]

\begin{lemma}\label{Suff}
If $X$ is a compact metric space, the following condition is sufficient for second weak shadowing: 
\[\forall \epsilon>0 \, \exists n \in \mathbb{N} \text{ s.t. } \forall x \in X \exists z \in X \text{ s.t. } \]
\[ \bigcup_{i=1} ^n B_{\frac{\epsilon}{3}}\left(f^i(x)\right) \supseteq \omega(z).\]
In particular, if the above condition is satisfied then, for any $\epsilon>0$ there is a $\delta>0$ such that the $\epsilon$-neighbourhood around every $\delta$-pseudo-orbit contains an $\omega$-limit set.
\end{lemma}

\begin{proof} Suppose that the condition given in the lemma is satisfied. Let $\epsilon>0$ be given and let $n \in \mathbb{N}$ be as in the condition with respect to $\epsilon$. We can use uniform continuity to choose $\delta>0$ such that every $\delta$-pseudo-orbit $\frac{\epsilon}{3}$-shadows the first $n$ iterates of its origin. Explicitly: Let $\delta_1>0$ be such that, for any $y, z \in X$, if $d(y,z) <\delta_1$ then $d(f(y),f(z)) < \frac{\epsilon}{3}$; without loss of generality $\delta_1 \leq \frac{\epsilon}{3}$. Now recursively, take $\delta_i>0$ for $i \in \{2,\ldots, n\}$, such that for any $y, z \in X$, if $d(y,z) <\delta_i$ then $d(f(y),f(z)) < \frac{\delta_{i-1}}{2}$ and such that $\delta_i < \frac{\delta_{i-1}}{2}$. Now pick $\delta \coloneqq \delta_n$. Suppose $(x_i)_{i \in \omega}$ is a $\delta$-pseudo-orbit. By the triangle inequality, $d(f^i(x_0),x_i) <\frac{\epsilon}{3}$ for all $i \in \{0, \ldots n\}$. By the given condition there exists $z \in X$ such that 
\[ \bigcup_{i=1} ^n B_{\frac{\epsilon}{3}}\left(f^i(x_0)\right) \supseteq \omega(z).\]
Therefore, by the triangle inequality, 
\[ \bigcup_{i=1} ^n B_{\frac{2\epsilon}{3}}\left(x_i\right) \supseteq \omega(z).\]
Since $\omega(z) \neq \emptyset$ as $X$ is compact, and since $\omega$-limit sets are positively invariant, the result follows.
\end{proof}


\begin{lemma}\label{Every}
If $X$ is a compact metric space, $(X,f)$ satisfies the following:
\[\forall \epsilon>0 \, \forall x \in X \exists n \in \mathbb{N} \exists z \in X \text{ s.t. } \]
\[ \bigcup_{i=1} ^n B_{\frac{\epsilon}{3}}\left(f^i(x)\right) \supseteq \omega(z).\]

\end{lemma}

\begin{proof} Take $\epsilon>0$ and pick $x \in X$. Take a finite subcover of the open cover $\{B_{\frac{\epsilon}{9}}(y) \mid y \in \omega(x)\}$ of $\omega(x)$. For each element of this subcover there exists $n$ such that $f^n(x)$ lies inside it. Pick one such $n$ for each element and then take the largest. The result follows by the triangle inequality.
\end{proof}

\begin{lemma}\label{Imply}
The condition in Lemma \ref{Every} implies the condition in Lemma \ref{Suff} if $X$ is a compact space.
\end{lemma}

\begin{proof}
Fix $\epsilon>0$. For each $x \in X$ let $n_x \in \mathbb{N}$ be as in the condition in Lemma \ref{Every} for $\frac{\epsilon}{3}$ and let $\delta_x>0$ be such that if $d(x,y) <\delta_x$ then, for each $i \in \{0,\ldots, n_x\}$, $d(f^i(x), f^i(y)) < \frac{\epsilon}{9}$. The collection $\{B_{\delta_x}(x) \mid x \in X\}$ forms an open cover. Let
\[\left\{B_{\delta_{x_i}}(x_i)\mid i \in \{1,\ldots, k\}\right\},\]
be a finite subcover. Take $n = \max_{i \in \{1, \ldots, k\}} n_{x_i}$. Then, by the triangle inequality, for any $x \in X$ there exists $z \in X$ such that 
\[\bigcup _{i=1} ^n B_\frac{\epsilon}{3}
\left(f^i(x)\right) \supseteq \omega(z). \]
\end{proof}

Using the above results, we can now show that every pseudo-orbit traps an $\omega$-limit set in its neighbourhood after a universal finite period of time.

\begin{theorem}\label{thmOmega}
Let $(X,f)$ be a dynamical system where $X$ is a compact space. Then for any $\epsilon>0$ 
there exist $n \in \mathbb{N}$ and $\delta>0$ such that given any $\delta$-pseudo orbit 
$(x_i)_{i \in \omega}$ there exists $z\in X$ such that
\[B_\epsilon\left((x_i)_{i=0} ^n \right) \supseteq \omega(z).\]
In particular,
\[B_\epsilon\left((x_i)_{i \in \omega}\right) \supseteq \omega(z).\]
\end{theorem}

\begin{proof}
As $X$ is compact it satisfies the condition in Lemma \ref{Every}, which, by Lemma \ref{Imply}, implies the condition in Lemma \ref{Suff} is also satisfied. By Lemma \ref{Suff}, the result holds.
\end{proof}

\begin{corollary}\label{CorOrbTrap}
Let $(X,f)$ be a dynamical system where $X$ is a compact metric space. Then the system has second weak shadowing.
\end{corollary}
\begin{proof}
This follows immediately from Theorem \ref{thmOmega}.
\end{proof}

Using these results we can draw out a corollary relating to the \textit{orbital shadowing property} as discussed in \cite{Pilugin2007,PiluginRodSakai2002}. Given a compact metric space $(X,d)$, the collection of compact subsets of $X$ form a metric space in their own right with the \textit{Hausdorff metric} induced by $d$; if $A$ and $B$ are compact subsets of $X$ then the \textit{Hausdorff distance} between $A$ and $B$ is given by
\[d_H(A,B) = \max \left\{ \sup_{a\in A}\inf_{b \in B}d(a,b), \sup_{b\in B} \inf_{a\in A}d(a,b)\right\}.\]
A dynamical system $(X,f)$ has the orbital shadowing property if, for any $\epsilon>0$ there exists $\delta>0$ such that for any $\delta$-pseudo-orbit $(x_i)_{i\in\omega}$, there exists a point $z$ with
\[d_H\left(\overline{\{x_i\}_{i \in \omega}}, \overline{\Orb(z)}\right) <\epsilon.\]
The second weak shadowing property discussed earlier is a weakening of the orbital shadowing property.

In \cite{GoodMeddaugh2016} the authors introduced the following strengthening of orbital shadowing which they demonstrate to be distinct.
\begin{definition}
Let $X$ be a compact metric space. A dynamical system $(X,f)$ has the \textit{strong orbital shadowing }property provided that for any $\epsilon>0$ there exists $\delta>0$ such that for any $\delta$-pseudo-orbit $(x_i)_{i\in\omega}$, there exists a point $z$ with
\[d_H\left(\overline{\{x_{N+i}\}_{i \in \omega}}, \overline{\{f^{N+i}(z)\}_{i \in \omega}}\right) <\epsilon,\]
for any $N \in \omega$.
\end{definition}
%Informally this means that the sets given by ignoring the same finite number of points from the beginning of each set are also $\epsilon$-close. 
When $X$ is a compact metric space we say a dynamical system $(X,f)$ is \textit{minimal} if $\omega(x)=X$ for each $x \in X$. 

%{\it This definition ($\omega$-limit set) must be before Lemma~\ref{Suff}. Sergio}
\begin{theorem}
Let $X$ be a compact metric space. If $(X,f)$ is a minimal dynamical system then it exhibits the strong orbital shadowing property.
\end{theorem}
\begin{proof}
Let $\epsilon>0$ be given. Take $\delta>0$ corresponding to $\epsilon$ as in Theorem \ref{thmOmega}. Now let $(x_i)_{i \in \omega}$ be a $\delta$-pseudo-orbit and take $z \in X$ such that
\[B_\epsilon\left((x_i)_{i\in \omega} \right) \supseteq \omega(z).\]
Because $(X,f)$ is minimal $\omega(x)=X$ for any $x \in X$; in particular $\omega(z)=X$. It follows that
\[B_\epsilon\left((x_i)_{i\in \omega} \right)=X.\]
Since the $\delta$-pseudo-orbit $(x_i)_{i\in \omega}$ was picked arbitrarily, this holds for any $\delta$-pseudo-orbit. In particular, for any $N \in \omega$, and any $x \in X$,
\[B_\epsilon\left((x_{N+i})_{i\in \omega}\right) =X.\]
It remains to remark that by definition, for any $x \in X$ and $N \in \omega$, $\omega(x) \subseteq \overline{\{f^{N+i}(x)\}_{i \in \omega}}$. Hence
\[d_H\left(\overline{\{x_{N+i}\}_{i \in \omega}}, \overline{\{f^{N+i}(x)\}_{i \in \omega}}\right) <\epsilon,\]
for any $N \in \omega$ and any $x \in X$.
\end{proof}

==> Sections/Graveyard/InverseShadowing.tex <==
\section{Inverse Shadowing}
Let $X$ be a compact metric space, and let $f \colon X \to X$ be a continuous onto function. A $\delta$-pseudo orbit is a sequence $(x_k)_{k\in \omega}$  such that $d(f(x_k), x_{k+1}) < \delta$ for all $k \in \omega$. Let $X^\omega$ be the product space of all mono-infinite sequences, with the product topology. For any given $\delta>0$, let $\Phi_f(\delta) \subseteq X^\omega$ be the set of all $\delta$-pseudo orbits. We call a mapping $\varphi \colon X \to \Phi_f(\delta)$, such that, for each $x \in X$, $\varphi_0(x)=x$, a $\delta$-method for $f$. We denote by $\mathcal{T}_0(f, \delta)$ the set of all $\delta$-methods.

\begin{definition}
Let $f \colon X \to X$ be a continuous onto function. We say that $f$ experiences $\mathcal{T}_0$-inverse shadowing if, for any $\epsilon>0$ there exists $\delta>0$ such that for any $x \in X$ and any $\varphi \in \mathcal{T}_0$ there exists $y \in X$ such that $\varphi(y)$ $\epsilon$-shadows $x$; i.e.
\[ \forall k \in \omega \colon d(\varphi_k(y), f^k(x))< \epsilon.\]
\end{definition}

Several authors (see \cite{Lee2} and \cite{Cor}) have commented on the fact that, when considering inverse shadowing, it is important to restrict one's attention to certain admissible classes of pseudo-orbits. We prove a lemma which brings to light exactly why such a restriction may be important; it shows that $\mathcal{T}_0$-inverse shadowing is much stronger than it might have seemed \textit{prima facie}.

\begin{lemma}\label{Reform}
A map $f\colon X \to X$ has $\mathcal{T}_0$ inverse shadowing if and only if for any $\epsilon>0$ there exists $\delta>0$ such that for any $x \in X$ there exists $y \in X$ such that for any $\varphi \in \mathcal{T}_0(f,\delta)$ and any $k \in \omega$ we have $d(f^k(x),\varphi(y)_k)<\epsilon$.
\end{lemma}

\begin{proof}
Clearly the latter implies the former. Thus, suppose $f$ has $\mathcal{T}_0$-inverse shadowing. Suppose the latter is false, i.e. there exists $\epsilon>0$ such that
\begin{equation}\label{eqnIS0.1}
\forall \delta>0 \exists x \in X \colon \forall y \in X \, \exists\varphi \in \mathcal{T}_0(X,f) \, \exists k \in \omega \colon d(f^k(x), \varphi(y)_k)\geq \epsilon.
\end{equation}
Take such an $\epsilon$. Then let $\delta>0$ correspond to this $\epsilon$ in the definition of inverse shadowing. Let $x \in X$ correspond to this $\epsilon$ and $\delta$ as in (\ref{eqnIS0.1}). Then, for any $y \in X$ there exists $\varphi \in  \mathcal{T}_0(X,f)$ and $k \in \omega$. For each $y \in X$, let $\varphi_y \in \mathcal{T}_0(X,f)$ be such a method. Then define a map $\varphi \colon X \to X^\omega \colon y \mapsto \varphi_y(y)$. By construction, $\varphi \in \mathcal{T}_0(X,f)$. By $\mathcal{T}_0$-inverse shadowing, there exists $y \in X$ such that $d(f^k(x),\varphi(y)_k)<\epsilon$ for all $k \in \omega$. But by construction, for this $y$, there exists $k \in \omega$ such that $d(f^k(x),\varphi(y)_k) \geq \epsilon$; a contradiction.
\end{proof}

\begin{lemma}\label{ReformCtd} Let $X$ be a compact metric space. A map $f\colon X \to X$ has $\mathcal{T}_0$-inverse shadowing if and only if for any $\epsilon>0$ there exists $\delta>0$ such that for any $x \in X$ there exists $y \in X$ such that for any $\varphi \in \mathcal{T}_0(f,\delta)$ and any $k \in \omega$ and any $z \in B_\delta(y)$, $d(f^k(x),\varphi(z)_k)<\epsilon$.
\end{lemma}

\begin{proof}
That the latter entails the former is trivial. Therefore, suppose the former. Let $\epsilon>0$ be given. Then, by Lemma \ref{Reform} there exists $\eta>0$ such that for any $x \in X$ there exists $y \in X$ such that for any $\varphi \in \mathcal{T}_0(f,\eta)$ and any $k \in \omega$ we have $d(f^k(x),\varphi(y)_k)<\frac{\epsilon}{2}$. Without loss of generality, $\eta<\frac{\epsilon}{2}$ Pick $x \in X$ and take $y \in X$ as given by Lemma \ref{Reform}. Using uniform continuity, take $\delta>0$ such that, for any $a,b \in X$, if $d(a,b)<\delta$ then $d(f(a),f(b)) < \frac{\eta}{2}$. Without loss of generality $\delta<\frac{\eta}{2}$. Now let $(z_k)_{k \in \omega}$ a $\delta$-pseudo orbit where $z_0 \in B_\delta(y)$. Then, by the triangle-inequality, $(y, z_1, \ldots, z_k, \ldots)$ is a $\eta$-pseudo orbit through $y$. It follows by the choice of $y$ that $d(f^k(x),z_k)<\frac{\epsilon}{2}$ for all $k \in \omega\setminus\{0\}$. Since \[d(x,z_0) < d(x,y)+d(y, z_0)<\frac{\epsilon}{2}+\delta<\frac{\epsilon}{2}+\eta<\epsilon,\] the sequence $(z_k)_{k \in \omega}$ $\epsilon$-shadows $x$ and we are done.
\end{proof}

In particular, Lemma \ref{ReformCtd} means that given any point and any $\epsilon>0$ there is an open set which $\epsilon$-shadows that point.

In \cite{Honour} the authors show a homeomorphism with $\mathcal{T}_0$-inverse shadowing is not expansive. We provide a stronger result.

\begin{theorem}
If $(X,d)$ is a metric space and a continuous onto map $f\colon X \to X$ has the $\mathcal{T}_0$-inverse shadowing property then the system $(X,f)$ is not eventually sensitive.
\end{theorem}

\begin{proof}
Suppose $f$ is eventually sensitive; let $\delta_0>0$ be a constant of eventual sensitivity. Pick $\epsilon>0$ with $\epsilon< \frac{\delta_0}{2}$. Now take a $\delta>0$ corresponding to this $\epsilon$ as in positive inverse shadowing. Pick $x \in X$; then there exists $y \in X$ such that every $\delta$-pseudo orbit through $y$ $\epsilon$-shadows $x$. Consider $f(y)$. Then, by eventual sensitivity there exists $n,k \in \mathbb{N}$ and there exists $z \in B_\delta\left(f^{n+1}(y)\right)$ such that $d(f^k(z), f^{n+k+1}(y))\geq \delta_0$. But the sequence 
\[(y,f(y),\ldots, f^{n}(y), z, f(z), \ldots f^k(z), f^{k+1}(z), \ldots),\]
is a $\delta$-pseudo orbit from $y$. Similarly so is the orbit sequence of $y$. Therefore, by inverse shadowing, $f^{n+k+1}(y),f^k(z) \in B_\epsilon\left(f^{n+k+1}(x)\right)$. It follows by the triangle inequality that
\[d\left(f^{n+k+1}(y),f^k(z)\right) < 2\epsilon < \delta_0,\]
a contradiction. Therefore $f$ is not eventually sensitive.
\end{proof}



\begin{definition}
A system $(X,f)$ exhibits finite $\mathcal{T}_0$-inverse shadowing if for any $\epsilon>0$ there exists $\delta>0$ such that for any $x \in X$ and any $\varphi \in \mathcal{T}_0(f,\delta)$ and any $n \in \mathbb{N}$ there exists $y_n \in X$ such that for any $k \in \{ 0, \ldots, n\}$ we have $d(f^k(x),\varphi(y_n)_k)<\epsilon$.
\end{definition}

The proof of the lemma below is very similar to that of Lemma \ref{Reform} and is thereby omitted.

\begin{lemma}\label{ReformFinite}
A map $f\colon X \to X$ has finite $\mathcal{T}_0$-inverse shadowing if and only if for any $\epsilon>0$ there exists $\delta>0$ such that for any $x \in X$ and any $n \in \mathbb{N}$ there exists $y_n \in X$ such that for any $\varphi \in \mathcal{T}_0(f,\delta)$ and any $k \in \{0, \ldots, n\}$ we have $d(f^k(x),\varphi(y)_k)<\epsilon$.
\end{lemma}

The following result shows that we only need to consider, and shadow, finite segments of orbits; this is likely to be helpful when proving more difficult results.

\begin{proposition}\label{Finite} Let $X$ be a compact metric space. A continuous onto map $f \colon X \to X$ has finite $\mathcal{T}_0$-inverse shadowing if and only if it has $\mathcal{T}_0$-inverse shadowing.
\end{proposition}

\begin{proof}
Clearly, if $f$ has it has $\mathcal{T}_0$-inverse shadowing then it has finite $\mathcal{T}_0$-inverse shadowing.

Suppose $f \colon X \to X$ has finite $\mathcal{T}_0$-inverse shadowing. Let $\epsilon>0$ be given and let $2\delta>0$ correspond to $\frac{\epsilon}{2}$ in finite inverse shadowing; wlog $\delta < \frac{\epsilon}{4}$. Then, by Lemma \ref{Reform}, for any $n \in \mathbb{N}$ there exists $y_n \in X$ such that for any $\varphi \in \mathcal{T}_0(f,2\delta)$, and any $i \in \{0,\ldots, n\}$, $d(\varphi(y_n)_i, f^i(x))< \frac{\epsilon}{2}$. By sequential compactness, $(y_n)$ has a convergent subsequence; call it $(y_n)$ again. Let $y=\lim_{n\to \infty} y_n$; $y \in \overline{B_{\frac{\epsilon}{2}}(x)}$. Because $f$ is continuous there exists $N \in \mathbb{N}$ such that $d(f(y_n),f(y))<\delta$ for all $n>N$. Then for any $n>N$ we have

\[B_\delta\left(f(y)\right)\subseteq B_{2\delta}\left(f(y_n)\right)\subseteq B_{\frac{\epsilon}{2}}\left(f(x)\right). \]

Now let $(z_k)_{k\in \omega}$ be a $\delta$-pseudo orbit through $y$ (so $z_0=y$), we will show this $\epsilon$-shadows $x$. Fix $n>N$. Then $(y_n,z_1,z_2,\ldots,z_{k},\ldots)$ is a $2\delta$-pseudo orbit through $y_n$; by finite shadowing $d(f^i(x), z_i) \leq \frac{\epsilon}{2}$ for all $i \in \{1,\ldots, n\}$. Additionally, $d(x,z_0)\leq \frac{\epsilon}{2}<\epsilon$, as $z_0=y$. Since $n>N$ was arbitrary it follows that, for any $n>N$, $d(f^i(x), z_i) \leq \frac{\epsilon}{2}$ for all $i \in \{0,1,\ldots, n\}$. This in turn entails that $d(f^i(x), z_i) \leq \frac{\epsilon}{2}$ for all $i \in \omega$. As this was an arbitrary $\delta$-pseudo orbit through $y$ we are done.
\end{proof}



==> Sections/Graveyard/InverseShadowingBoth.tex <==
\section{Inverse Shadowing} \label{section-inverse}
Let $X$ be a compact metric space, and let $f \colon X \to X$ be a homeomorphism (resp. a continuous onto function). For this section a $\delta$-pseudo-orbit is a bi-infinite sequence $(x_k)_{k\in \mathbb{Z}}$  such that $d(f(x_k), x_{k+1}) < \delta$ for all $k \in \mathbb{Z}$. What were called $\delta$-pseudo-orbits in previous sections will now be referred to as positive $\delta$-pseudo-orbits. Let $X^\mathbb{Z}$ (resp. $X^\omega$) be the product space of all bi-infinite (resp. mono-infinite) sequences, with the product topology; note that this is compact metric. Then, for any given $\delta>0$, let $\Phi_f(\delta) \subseteq X^\mathbb{Z}$ be the set of all $\delta$-pseudo-orbits (resp. $\Phi ^+ _f(\delta) \subseteq X^\omega$ the set of all positive $\delta$-pseudo-orbits). We call a mapping $\varphi \colon X \to \Phi_f(\delta)$ (resp. $\varphi\colon X\to\Phi_f^+(\delta)$), such that, for each $x \in X$, $\varphi(x)_0=x$, a (resp. positive) $\delta$-method for $f$ where $\varphi(x)_k$ is used to denote the $k$th term in the sequence $\varphi(x)$. We denote by $\mathcal{T}_0(f, \delta)$ the set of all respective $\delta$-methods with understanding from the context whether this refers to positive methods or not. We denote by $\mathcal{T}_c(f,\delta)$ the set of all continuous (positive) $\delta$-methods, and by $\mathcal{T}_h(f,\delta)$ the set of all (positive) $\delta$-methods induced by a homeomorphism; i.e., $\mathcal{T}_h(f,\delta)$ is the set of (resp. positive) $\delta$-methods $\varphi$ for which there exists a homeomorphism $h \colon X \to X$ such that $d(f(x),h(x))< \delta$ for each $x \in X$ and $\varphi(x)_k=h^k(x)$, for all relevant $k \in \mathbb{Z}$ (resp. $k \in \omega$).


\begin{definition}
Let $f \colon X \to X$ be a homeomorphism (resp. continuous onto function). We say that $f$ experiences \textit{(resp. positive) $\mathcal{T}_\alpha$-inverse shadowing}
%\footnote{For positive $\mathcal{T}_\alpha$-inverse shadowing, the class $\mathcal{T}_\alpha$ is considered the collection of all relevant \textit{forward} $\delta$-methods. For example, if $\varphi \in \mathcal{T}_0$ then $\varphi(y)$ is a positive pseudo orbit starting from $y$.}
if, for any $\epsilon>0$ there exists $\delta>0$ such that for any $x \in X$ and any $\varphi \in \mathcal{T}_\alpha(f,\delta)$ there exists $y \in X$ such that $\varphi(y)$ $\epsilon$-shadows $x$; i.e.
\[ \forall k \in \mathbb{Z} \,( \textit{resp. } k \in \omega), \,d(\varphi(y)_k, f^k(x))< \epsilon.\]
\end{definition}

Several authors \cite{CorlessPilyugin, Lee} have commented on the fact that, when considering inverse shadowing, it is important to restrict one's attention to certain admissible classes of pseudo-orbits. We prove a result which brings to light exactly why such a restriction may be important; it shows that $\mathcal{T}_0$-inverse shadowing is much stronger than it might have seemed \textit{prima facie}.


\begin{theorem}\label{Reform}
A map $f\colon X \to X$ has (resp. positive) $\mathcal{T}_0$-inverse shadowing if and only if for any $\epsilon>0$ there exists $\delta>0$ such that for any $x \in X$ there exists $y \in X$ such that for any $\varphi \in \mathcal{T}_0(f,\delta)$ and any $k \in \mathbb{Z}$ (resp. $k \in \omega$) $d(f^k(x),\varphi(y)_k)<\epsilon$.
\end{theorem}

\begin{proof}
Clearly the latter implies the former. Thus, suppose that $f$ has (resp. positive) $\mathcal{T}_0$-inverse shadowing and assume further that the latter is false, that is, there exists an $\varepsilon>0$ such that
\begin{align}\label{eqnIS0.1}
\forall \delta>0 \exists x \in X : \forall y \in X \, \exists\varphi \in \mathcal{T}_0(f,\delta) \, \exists k \in \mathbb{Z} \, (\text{resp. } k \in \omega) : d(f^k(x), \varphi(y)_k)\geq \epsilon.
\end{align}


Take such an $\epsilon$ and let $\delta>0$ correspond to this $\epsilon$ in the definition of inverse shadowing. Now, fix $x \in X$ corresponding to this $\epsilon$ and $\delta$ as in (\ref{eqnIS0.1}). Then by (\ref{eqnIS0.1}), for each $y \in X$, there will exist a $\varphi_y \in \mathcal{T}_0(f,\delta)$ and a $k\in\mathbb{Z}$ (resp. $k\in\omega$) for which $d(f^k(x), \varphi_y(y)_k)\geq \epsilon$. Now, define a map $\varphi \colon X \to X^\mathbb{Z} \colon y \mapsto \varphi_y(y)$. By construction, $\varphi \in \mathcal{T}_0(f,\delta)$ and by (resp. positive) $\mathcal{T}_0$-inverse shadowing, there will exist $y \in X$ such that $d(f^k(x),\varphi(y)_k)<\epsilon$ for all $k \in \mathbb{Z}$ (resp. $k\in \omega)$. But by the construction of $\varphi$, this can not be the case for all such $k$ and thus one obtains a contradiction.
\end{proof}

\begin{lemma}\label{ReformCtd} Let $X$ be a compact metric space. A homeomorphism (resp. continuous onto map) $f\colon X \to X$ has (resp. positive) $\mathcal{T}_0$-inverse shadowing if and only if for any $\epsilon>0$ there exists $\delta>0$ such that for any $x \in X$ there exists $y \in X$ such that for any $\varphi \in \mathcal{T}_0(f,\delta)$ and any $k \in \mathbb{Z}$ (resp. $k \in \omega$)  and any $z \in B_\delta(y)$, $d(f^k(x),\varphi(z)_k)<\epsilon$.
\end{lemma}

\begin{proof}
That the latter entails the former is trivial. Therefore, suppose the former. Let $\epsilon>0$ be given. Then, by Theorem \ref{Reform} there exists $\eta>0$ (without loss of generality $\eta<\frac{\varepsilon}{2}$) such that for any $x \in X$, there exists $y \in X$ such that for any $\varphi \in \mathcal{T}_0(f,\eta)$ and any $k \in \mathbb{Z}$ (resp. $k \in \omega$) $d(f^k(x),\varphi(y)_k)<\frac{\epsilon}{2}$.

First consider the case when $f$ is a homeomorphism. Using uniform continuity, take $\delta>0$ such that, for any $a,b \in X$, if $d(a,b)<\delta$ then $d(f(a),f(b)) < \frac{\eta}{2}$ and $d(f^{-1}(a),f^{-1}(b))< \frac{\eta}{2}$; without loss of generality $\delta<\frac{\eta}{2}$. Now let $(z_k)_{k \in \mathbb{Z}}$ be a $\delta$-pseudo-orbit where $z_0 \in B_\delta(y)$. Then, by the triangle inequality, \[(\ldots, z_{-k},\ldots, z_{-1}, y, z_1, \ldots, z_k, \ldots)\] is a $\eta$-pseudo-orbit through $y$. It follows by the choice of $y$ that $d(f^k(x),z_k)<\frac{\epsilon}{2}$ for all $k \in \mathbb{Z}\setminus\{0\}$. Since $d(x,z_0) \leq d(x,y)+d(y, z_0)=\frac{\epsilon}{2}+\eta<\epsilon$, the sequence $(z_k)_{k \in \mathbb{Z}}$ $\epsilon$-shadows $x$ and we are done.

Now suppose that $f$ is a continuous onto map; we are now considering positive $\mathcal{T}_0$-inverse shadowing. We argue similarly to before. Using uniform continuity, take $\delta>0$ such that, for any $a,b \in X$, if $d(a,b)<\delta$ then $d(f(a),f(b)) < \frac{\eta}{2}$. Without loss of generality $\delta<\frac{\eta}{2}$. Now let $(z_k)_{k \in \omega}$ be a $\delta$-pseudo-orbit where $z_0 \in B_\delta(y)$. Then, by the triangle inequality, $(y, z_1, \ldots, z_k, \ldots)$ is a $\eta$-pseudo-orbit through $y$. It follows by the choice of $y$ that $d(f^k(x),z_k)<\frac{\epsilon}{2}$ for all $k \in \omega\setminus\{0\}$. Since \[d(x,z_0) \leq d(x,y)+d(y, z_0)<\frac{\epsilon}{2}+\delta<\frac{\epsilon}{2}+\eta<\epsilon,\] the sequence $(z_k)_{k \in \omega}$ $\epsilon$-shadows $x$ and we are done.
\end{proof}


In particular, Lemma \ref{ReformCtd} means that given any point and any $\epsilon>0$ there is an open set which $\epsilon$-shadows that point.

In \cite{Honary} the authors show a homeomorphism with $\mathcal{T}_0$-inverse shadowing is not expansive. We provide a stronger result.

\begin{theorem}\label{thmInvShadNotEvSens}
If $(X,d)$ is a metric space and a continuous onto map $f\colon X \to X$ has the positive $\mathcal{T}_0$-inverse shadowing property then the system $(X,f)$ is not eventually sensitive. (If $f$ is a homeomorphism with $\mathcal{T}_0$-inverse shadowing, then neither $(X,f)$ nor the inverse system $(X,f^{-1})$ are eventually sensitive.)
\end{theorem}

\begin{proof}
Suppose that $f$ is eventually sensitive and let $\delta_0>0$ be a constant of eventual sensitivity. Pick $\epsilon>0$ with $\epsilon< \frac{\delta_0}{2}$. Now take a $\delta>0$ corresponding to this $\epsilon$ as in positive inverse shadowing. Choose $x \in X$; then there exists $y \in X$ such that every $\delta$-pseudo-orbit through $y$ $\epsilon$-shadows $x$. Consider $f(y)$. Then, by eventual sensitivity there exist $n,k \in \mathbb{N}$ and $z \in B_\delta\left(f^{n+1}(y)\right)$ such that $d(f^k(z), f^{n+k+1}(y))\geq \delta_0$. But the sequence 
\[(y,f(y),\ldots, f^{n}(y), z, f(z), \ldots f^k(z), f^{k+1}(z), \ldots),\]
is a $\delta$-pseudo orbit from $y$. Similarly so is the orbit sequence of $y$. Therefore, by inverse shadowing, $f^{n+k+1}(y),f^k(z) \in B_\epsilon\left(f^{n+k+1}(x)\right)$. It follows by the triangle inequality that
\[d\left(f^{n+k+1}(y),f^k(z)\right) < 2\epsilon < \delta_0,\]
which is a contradiction. Therefore $f$ is not eventually sensitive.
\end{proof}

\begin{definition}
Let $f \colon X \to X$ be a homeomorphism (resp. continuous onto function). We say that $f$ experiences \textit{(resp. positive) weak inverse shadowing} with respect to the class $\mathcal{T}_\alpha$ if, for any $\epsilon>0$ there exists $\delta>0$ such that for any $x \in X$ and any $\varphi \in \mathcal{T}_\alpha(f,\delta)$ there exists $y \in X$ such that 
\[\varphi(y) \subseteq B_\epsilon\left(\Orb(x)\right).\]
(Considering $\Orb(x)$ as both the forward and backward orbit of $x$ under $f$ in the case when $f$ is a homeomorphism.)
\end{definition}

\begin{remark}
Clearly if a system has $\mathcal{T}_\alpha$-inverse shadowing then it has weak inverse shadowing with respect to the class $\mathcal{T}_\alpha$.
\end{remark}

Using the same technique as in the proof of Theorem \ref{Reform} we come by the following reformulation of weak inverse shadowing.

\begin{lemma}\label{ReformWeak}
A map $f\colon X \to X$ has (resp. positive) weak inverse shadowing with respect to the class  $\mathcal{T}_0$ if and only if for any $\epsilon>0$ there exists $\delta>0$ such that for any $x \in X$ there exists $y \in X$ such that for any $\varphi \in \mathcal{T}_0(f,\delta)$, \[\varphi(y) \subseteq B_\epsilon\left(\Orb(x)\right).\]
(Considering $\Orb(x)$ as both the forward and backward orbit of $x$ under $f$ in the case when $f$ is a homeomorphism.)
\end{lemma}


In \cite{Honary} the authors show that a chain transitive homeomorphism is minimal if and only if it has the weak inverse shadowing property with respect to $\mathcal{T}_0$. With Lemma \ref{ReformWeak} this result, as well as the following analogous one, become much more elementary.

\begin{theorem}[\cite{Honary}]\label{thmInvShadTTEq}
Let $X$ be a compact metric space and $f \colon X \to X$ be a chain transitive continuous onto function. Then $f$ is minimal if and only if $f$ has positive weak inverse shadowing with respect to the class $\mathcal{T}_0$.
\end{theorem}

\begin{proof}
Since the orbit of every point is dense under a minimal map, it is trivial that such a map has positive weak inverse shadowing with respect to the class $\mathcal{T}_0$.

Pick $z \in X$. Let $\epsilon>0$ and take $\delta>0$ as in Lemma \ref{ReformWeak}. Then there exists $y \in X$ such that for any $\varphi \in \mathcal{T}_0(f,\delta)$, \[\varphi(y) \subseteq B_\epsilon\left(\Orb(z)\right).\]
Since $f$ is chain transitive there is a $\delta$-chain from $y$ to every point in $X$. It follows then by the above that $x \in B_\epsilon\left(\Orb(z)\right)$ for all $x \in X$. Since $\epsilon>0$ was arbitrary the result follows. 
\end{proof}


\begin{corollary}
Let $X$ be a compact metric space and let $f \colon X \to X$ be a chain transitive continuous onto function. Then, if $f$ has the positive $\mathcal{T}_0$-inverse shadowing property then the system $(X,f)$ is equicontinuous. (If $f$ is a homeomorphism with $\mathcal{T}_0$-inverse shadowing, then both $(X,f)$ and the inverse system $(X,f^{-1})$ are equicontinuous.)
\end{corollary}
\begin{proof}
By Theorem \ref{thmInvShadTTEq} $(X,f)$ is a transitive system. A transitive system is either equicontinuous or eventually sensitive (see \cite{GoodLeekMitchell}). The result now follows from Theorem \ref{thmInvShadNotEvSens}.
\end{proof}


As previously mentioned, shadowing is equivalent to finite shadowing in a compact system  \cite{PiluginRodSakai2002}. We provide a similar result for inverse shadowing with respect to each of the classes $\mathcal{T}_\alpha$.


\begin{definition}
A system $(X,f)$ exhibits \textit{finite (resp. finite positive) $\mathcal{T}_\alpha$-inverse shadowing} if for any $\epsilon>0$ there exists $\delta>0$ such that for any $x \in X$ and any $\varphi \in \mathcal{T}_0(f,\delta)$ and any $n \in \mathbb{N}$ there exists $y_n \in X$ such that for any $k \in \{-n,\ldots, 0, \ldots, n\}$ (resp. $k \in \{0, \ldots, n\}$) $d(f^k(x),\varphi(y_n)_k)<\epsilon$.
\end{definition}

The proof of the lemma below is very similar to that of Lemma \ref{Reform} and is therefore omitted.

\begin{lemma}\label{ReformFinite}
A map $f\colon X \to X$ has finite (resp. finite positive) $\mathcal{T}_0$-inverse shadowing if and only if for any $\epsilon>0$ there exists $\delta>0$ such that for any $x \in X$ and any $n \in \mathbb{N}$ there exists $y_n \in X$ such that for any $\varphi \in \mathcal{T}_0(f,\delta)$ and any $k \in \{-n,\ldots, 0, \ldots, n\}$ (resp. $k \in \{0, \ldots, n\}$) $d(f^k(x),\varphi(y)_k)<\epsilon$.
\end{lemma}

The following result states that finite inverse shadowing, for any given class, is equivalent to inverse shadowing, for that same class. It is analogous to the previously mentioned result that, on a compact space, shadowing is equivalent to finite shadowing \cite{Pilyugin}.

\begin{proposition}\label{Finite} Let $X$ be a compact metric space. For any $\alpha \in \{0,c,h\}$, a homeomorphism (resp. continuous onto map) $f \colon X \to X$ has finite (positive) $\mathcal{T}_\alpha$-inverse shadowing if and only if it has (positive) $\mathcal{T}_\alpha$-inverse shadowing.
\end{proposition}

\begin{proof}
We will prove the cases when $f$ is a homeomorphism, with reference to $\mathcal{T}_\alpha$-inverse shadowing. The cases when $f$ is a continuous onto map, with reference to positive $\mathcal{T}_\alpha$-inverse shadowing, are similar.

Clearly, for any $\alpha \in \{0,c,h\}$, if $f$ has it has (positive) $\mathcal{T}_\alpha$-inverse shadowing then it has finite (positive) $\mathcal{T}_\alpha$-inverse shadowing.

Suppose that $f \colon X \to X$ has finite $\mathcal{T}_c$-inverse shadowing. Let $\epsilon>0$ be given and let $\delta>0$ correspond to $\frac{\epsilon}{2}$ in finite inverse shadowing. Let $x\in X$ and take $\varphi \in \mathcal{T}_c(f,\delta)$. For any $n \in \mathbb{N}$, there exists $y_n\in X$ such that $d(\varphi(y_n)_i,f^i(x))<\frac{\epsilon}{2}$ for all $i \in \{-n \ldots, 0, \ldots, n\}$. By sequential compactness, $(y_n)$ has a convergent subsequence; call it $(y_n)$ again. Let $y=\lim_{n\to \infty} y_n$; $y \in \overline{B_{\frac{\epsilon}{2}}(x)}$. Since $\varphi \colon X \to X^\mathbb{Z}$ is continuous, 
\[\lim_{n\to \infty}\varphi(y_n)=\varphi\left(\lim_{n\to \infty}y_n\right)=\varphi(y).\]
Moreover it follows that, for any $k \in \mathbb{N}$ there exists $M \in \mathbb{N}$ such that for any $m>M$ we have $d(\varphi(y)_i, \varphi(y_m)_i)<\frac{\epsilon}{2}$ for all $i \in \{-k, \ldots, 0, \ldots, k\}$. For a fixed $k$ and corresponding $M$, we must also have, for all $m>M$ that, $d(\varphi(y_m)_i,f^i(x))<\frac{\epsilon}{2}$ for all $i \in \{-k, \ldots, 0, \ldots, k\}$. Then, by the triangle inequality,

\[\forall k \in \mathbb{N} \exists M \in \mathbb{N} : \forall m>M \, \forall i \in \{-k, \ldots, 0, \ldots, k\}, \, d(\varphi(y)_i, f^i(x))<\epsilon.\]
From this it follows that for every $k \in \mathbb{N}$ we have $d(\varphi(y)_k, f^k(x))<\epsilon$.
Hence $f \colon X \to X$ has $\mathcal{T}_c$-inverse shadowing. The proof for the class $\mathcal{T}_h$ is similar to the above (as are the positive versions for the classes $\mathcal{T}_c$ and $\mathcal{T}_h$); these are therefore omitted.

Now suppose that $f \colon X \to X$ has finite $\mathcal{T}_0$-inverse shadowing. Let $\epsilon>0$ be given and let $2\delta>0$ correspond to $\frac{\epsilon}{2}$ in finite inverse shadowing; without loss of generality taking $\delta < \frac{\epsilon}{4}$. Then, by Lemma \ref{Reform}, for any $n \in \mathbb{N}$ there exists $y_n \in X$ such that for any $\varphi \in \mathcal{T}_0(f,2\delta)$, and any $i \in \{-n, \ldots,0,\ldots, n\}$, $d(\varphi(y_n)_i, f^i(x))< \frac{\epsilon}{2}$. By sequential compactness, $(y_n)$ has a convergent subsequence; call it $(y_n)$ again. Let $y=\lim_{n\to \infty} y_n$; $y \in \overline{B_{\frac{\epsilon}{2}}(x)}$. Because $f$ and $f^{-1}$ are continuous, there exists $N \in \mathbb{N}$ such that $d(f(y_n),f(y))<\delta$ and $d(f^{-1}(y_n),f^{-1}(y))<\delta$ for all $n>N$. Then for any $n>N$ we have

\[B_\delta\left(f(y)\right)\subseteq B_{2\delta}\left(f(y_n)\right)\subseteq B_{\frac{\epsilon}{2}}\left(f(x)\right), \]
and
\[B_\delta\left(f^{-1}(y)\right)\subseteq B_{2\delta}\left(f^{-1}(y_n)\right)\subseteq B_{\frac{\epsilon}{2}}\left(f^{-1}(x)\right). \]

Now let $(z_k)_{k\in \mathbb{Z}}$ be a $\delta$-pseudo-orbit through $y$ (so $z_0=y$), we will show this $\epsilon$-shadows $x$. Fix $n>N$. Then \[(\ldots,...,z_{-k},\ldots,z_{-2}, z_{-1},y_n,z_1,z_2,\ldots,z_{k},\ldots),\] is a $2\delta$-pseudo-orbit through $y_n$; by finite shadowing $d(f^i(x), z_i) \leq \frac{\epsilon}{2}$ for all $i \in \{-n,\ldots, -1,1,\ldots, n\}$. Additionally, $d(x,z_0)\leq \frac{\epsilon}{2}<\epsilon$, as $z_0=y$. Since $n>N$ was arbitrary it follows that, for any $n>N$, $d(f^i(x), z_i) \leq \frac{\epsilon}{2}$ for all $i \in \{-n,\ldots, -1,1,\ldots, n\}$. This in turn entails that $d(f^i(x), z_i) \leq \frac{\epsilon}{2}$ for all $i \in \mathbb{Z}$. As this was an arbitrary $\delta$-pseudo-orbit through $y$ we are done.
\end{proof}


==> Sections/Graveyard/Questions_to_consider.tex <==
\section{Questions}
\begin{enumerate}
\item unique limit iff limit and no asymptotic pairs. NB. implies 1-1.  +ve expansive plus unique limit implies homoemorphism so finite.  What about +ve 2-expansive 
\item 2-sided limit shadopwing with gap
\item unique 2-sided limit shadowing
\item unique s-limit shadowing and c-expansive (equiv. unique two-sided shadowing) iff unique two-sided-s-limit.??
\item unique shad implies unique h-shadowing. CHECK converse. 
\item unique eventual shadowing implies 1 to 1 and non asymptotic pairs.  Relate to unique limit.  HEnce finite if +ve expansive.
\item unique orbital
\item unique strong orbital;
\item unique inverse
\item unique ergodic iff unique shadowing plus mixing/transitive?  
\item unique specification
\item unique ramsey 
\item unique anything else that makes sense
\item not quite 1-1 but global $\epsilon$ such that if closer than this it is one to one.
\item Carvalho Cordiero n-expansive, talks about limit shadowing from unique shadowing do we hav a generalization?
\item L-shaodwing, expansivity, s-limit, two sideds s-limit.  Our n-expanisve example has two sided s-limit.
\item (+ve) 2-expansive + shadowing implies (2) s-limit shadowing?
\item +ve 2-expansive homeo implies finite?
\item +ve 2-expansive open implies shadowing?? cf Sakai +ve expansive open implies shadowing  
\end{enumerate}

QUESTION: What about uniqueness of other forms of shadowing? limit, s-limit etc etc, two sided limit shadowing, Specification property?  Converse? others

We have unique limit shadowing iff limit shadowing plus no asymptotic pairs.

==> Sections/Graveyard/slimit_Shadowing.tex <==
\section{s-limit shadowing} \label{section-s-limit}

\begin{definition}
The system $(X, f)$ is said to have \textit{limit shadowing} if every asymptotic pseudo-orbit is asymptotically shadowed.
\end{definition}

The definition of limit shadowing was extended in \cite{LeeSakai} to a property the authors called s-limit shadowing. This was done to accommodate the fact that many systems exhibit limit shadowing but not shadowing \cite{Kulczycki,Pilyugin}.

\begin{definition}
The system $(X, f)$ is said to have \textit{s-limit shadowing }if for any $\epsilon >0$ there exists $\delta >0$ such that the following two conditions hold: 
\begin{enumerate}
\item every $\delta$-pseudo orbit is $\epsilon$-shadowed, and
\item every asymptotic $\delta$-pseudo orbit is asymptotically $\epsilon$-shadowed.
\end{enumerate}
\end{definition}

For a large class of studied systems, it turns out that this definition can be made more compact.


\begin{theorem}
If $X$ is a compact metric space then condition (1) in the definition of s-limit shadowing is obsolete.
\end{theorem}

\begin{proof}
Condition (1) simply says that part of what it means for a system to have s-limit 
shadowing is that it has shadowing. Recall from Section \ref{section-shadowing}, for a compact metric 
system the notion of shadowing is equivalent to that of finite shadowing. Now, suppose that 
$(X,f)$ satisfies condition (2). Let $\epsilon>0$ be given and take a corresponding $\delta$. 
Let $(x_0,x_1,\ldots, x_m)$ be a finite $\delta$-pseudo orbit. Then
\[(x_0, x_1, \ldots, x_m, f(x_m), f^2(x_m), \ldots, f^k(x_m), \ldots),\]
is an asymptotic $\delta$-pseudo orbit. By condition \textit{(2)} this is 
asymptotically $\epsilon$-shadowed by a point, say $x$. In particular 
$d(f^i(x),x_i) < \epsilon$ for all $i \in \{0,1, \ldots, m\}$; hence $(X,f)$ has finite shadowing.
\end{proof}

DOES 2-sided limit shadowing imply 2 sided s-limit shadowing?

==> Sections/UniqueTypes/Unique_h-shadowing.tex <==
\subsection{Unique h-shadowing}

\begin{definition}
Let $(X,f)$ be a dynamical system. The map $f$ has \emph{unique h-shadowing} if there exists $\eta>0$ such that for any $\epsilon>0$ there exists $\delta>0$ such that for any finite $\delta$-pseudo-orbit $(x_0, \ldots , x_n)$ there exists a unique point $z$ such that $d(f^i(z), x_i) < \epsilon$ for each $i \in \{0, \ldots, n\}$ and $f^n(z)=x_n$.
\end{definition}


\begin{theorem}\label{thmUniqueShadImpliesUnique_h-shad} Let $(X,f)$ be a dynamical system. If $f$ has unique shadowing then it has unique h-shadowing.
\end{theorem}
\begin{proof}
Suppose that $f$ has unique shadowing: let $\eta>0$ be as in the condition for this and let $\epsilon>0$ be arbitrary. Let $\delta_0$ correspond to $\epsilon$ for unique shadowing. By Corollary \ref{corollaryUniqueshad_hshad_limitshad_s-lim_shad}, $f$ has h-shadowing. Let $\delta>0$ be such that $\delta<\delta_0$ and satisfy the property of h-shadowing with respect to $\epsilon$. Let $(x_0, \ldots, x_n)$ be a finite $\delta$-pseudo-orbit. Extend this into a $\delta$-pseudo-orbit $(x_i)_{i\geq 0}$ by taking $x_{n+m}=f^m(x_n)$ for all $m \in \mathbb{N}$. By h-shadowing there exists $z \in X$ such that $d(f^i(z), x_i)< \epsilon$ for all $i \in \mathbb{N}_0$ and $f^n(z)=x_n$. Let $y \in X$ also have this property (we will show $y=z$). It follows immediately that $y$ and $z$ $\epsilon$-shadow $(x_i)_{i \geq 0}$. By unique shadowing we therefore have $y=z$.
\end{proof}

The converse to Theorem \ref{thmUniqueShadImpliesUnique_h-shad} is false as shown by the following example.

\begin{example}\label{example_Unique_h_shad_not_unique_shad} Consider $X= \{1/2^n \mid n \in \mathbb{N}_0\} \cup \{0\}$ and let $f$ be the identity map on $X$. Then $f$ has unique h-shadowing but, by Corollary \ref{corollaryUniqueshad_hshad_limitshad_s-lim_shad}, not unique shadowing because it is not positively expansive.
\end{example}

==> Sections/UniqueTypes/Unique_limit_shad.tex <==
\subsection{Unique limit shadowing}

\begin{definition} Let $(X,f)$ be a dynamical system. The map $f$ has \emph{unique limit shadowing} if every asymptotic pseudo-orbit is asymptotically shadowed by a unique point.
\end{definition}

We say a pair $(x,y) \in X \times X$ is \emph{asymptotic} if \[\lim_{n\rightarrow \infty} d(f^n(x),f^n(y))=0.\]


\begin{theorem} Let $(X,f)$ be a dynamical system. The map $f$ has unique limit shadowing if and only if it has limit shadowing and no asymptotic pairs.
\end{theorem}
\begin{proof}
If $f$ has unique limit shadowing then it has limit shadowing. Furthermore, since every point asymptotically shadows the asymptotic pseudo-orbit given by its own forward orbit, uniqueness ensures no asymptotic pairs.

Now suppose $f$ has limit shadowing and no asymptotic pairs. Let $(x_i)_{i \in \mathbb{N}_0}$ be an asymptotic pseudo-orbit. If this is asymptotically shadowed by $y,z \in X$ then $\lim_{i \to \infty} d(f^i(y), f^i(z)) =0$: thus $y=z$ since there are no asymptotic pairs.
\end{proof}

\begin{corollary} If $(X,f)$ is a dynamical system with unique limit shadowing then it is injective.
\end{corollary}

==> Sections/UniqueTypes/Unique_s_limit_shadowing.tex <==
\subsection{Unique s-limit shadowing}
We close by examining the implications of uniqueness in other forms of shadowing, namely, s-limit, limit and h-shadowing.
\begin{definition}Let $(X,f)$ be a dynamical system. The map $f$ has \emph{unique s-limit shadowing} if
\begin{enumerate}
\item it has unique shadowing; and,
\item there exists $\eta>0$ such that for any $\epsilon>0$ with $\epsilon< \eta$ there exists $\delta>0$ such that every asymptotic $\delta$-pseudo-orbit is asymptotically $\epsilon$-shadowed by a unique point.
\end{enumerate}
\end{definition}

\begin{definition}Let $(X,f)$ be a dynamical system. The map $f$ has \emph{two-sided unique s-limit shadowing} if
\begin{enumerate}
\item it has two-sided unique shadowing; and,
\item there exists $\eta>0$ such that for any $\epsilon>0$ with $\epsilon< \eta$ there exists $\delta>0$ such that every two-sided asymptotic $\delta$-pseudo-orbit is two-sided asymptotically $\epsilon$-shadowed by a unique point.
\end{enumerate}
\end{definition}

\begin{remark}
It is easy to see that postulating uniqueness in condition (2) is rendered obsolete by condition (1). However, we also observe that condition (1) itself is rendered obsolete by condition (2), see \cite{GoodMitchellThomas}.
\end{remark}

Given Corollary \ref{corollaryUniqueshad_hshad_limitshad_s-lim_shad}, the following theorem is straightforward.

\begin{theorem}Let $(X,f)$ be a dynamical system. Then the map $f$ has
\begin{enumerate}
    \item unique shadowing if and only if it has unique s-limit shadowing.
    \item two-sided unique shadowing if and only if it has two-sided unique s-limit shadowing.
\end{enumerate}
\end{theorem}
\begin{proof}
(1): Clearly it will suffice to show unique shadowing implies unique s-limit shadowing. Therefore, suppose that the map $f$ has unique shadowing. Then $f$ has s-limit shadowing by Corollary \ref{corollaryUniqueshad_hshad_limitshad_s-lim_shad}. Let $\eta>0$ be as in the condition for unique shadowing. Now let $\epsilon>0$ be given, with $\epsilon<\eta$. By s-limit shadowing there exists $\delta>0$ such that every asymptotic $\delta$-pseudo-orbit is asymptotically $\epsilon$-shadowed. If there exists an asymptotic $\delta$-pseudo-orbit which is asymptotically $\epsilon$-shadowed by two or more distinct points then this would contradict the fact that the system has unique shadowing. 

The proof of (2) is similar.
\end{proof}


==> Sections/UniqueTypesOfShadowing.tex <==
\section{Uniqueness of other shadowing properties}

\input{Sections/UniqueTypes/Unique_s_limit_shadowing.tex}
\input{Sections/UniqueTypes/Unique_limit_shad.tex}
\input{Sections/UniqueTypes/Unique_h-shadowing.tex}
